Cosmoglobe DR2. I. Global Bayesian analysis of COBE-DIRBE

We present the first global Bayesian analysis of the time-ordered DIRBE data within the Cosmoglobe framework, building on the same methodology that has previously been successfully applied to Planck LFI and WMAP. These data are analyzed jointly with COBE-FIRAS, Gaia, Planck HFI, and WISE, allowing for more accurate instrumental and astrophysical characterization than possible through single-experiment analysis. This paper provides an overview of the analysis pipeline and main results, and we present and characterize a new set of zodiacal light subtracted mission average (ZSMA) DIRBE maps spanning 1.25 to 240 $\mu$m. A novel aspect of this processing is the characterization and removal of excess radiation between 4.9 and 60$\,\mu$m that appears static in solar-centric coordinates. The DR2 ZSMA maps have several advantages with respect to the previously available maps, including 1) lower zodiacal light (and possibly straylight) residuals; 2) better determined zero-levels; 3) natively HEALPix tessellated maps with a $7'$ pixel size; 4) nearly white noise at pixel scales; and 5) a more complete and accurate noise characterization established through the combination of MCMC samples and half-mission maps. In addition, because the model has been simultaneously fitted with both DIRBE and HFI data, this is the first consistent unification of the infrared and CMB wavelength ranges into one global sky model covering 100 GHz to 1 $\mu$m. However, even though the new maps are improved with respect to the official maps, and should be preferred for most future analyses that require DIRBE sky maps, they still exhibit non-negligible zodiacal light residuals between 12 and 60$\,\mu$m. Further improvements should be made through joint analysis with complementary infrared experiments such IRAS, AKARI, WISE and SPHEREx, and releasing the full combined potential of all these powerful infrared observatories.

==> detector_table.tex <==
\begin{table*}[t]
  \begingroup
  \newdimen\tblskip \tblskip=5pt
	\caption{List of detector properties (from \citealt{silverberg93} Table 2).}
  \label{tab:detectors}
  \nointerlineskip
  \vskip -3mm
  \footnotesize
  \setbox\tablebox=\vbox{
    \newdimen\digitwidth
    \setbox0=\hbox{\rm 0}
    \digitwidth=\wd0
    \catcode`*=\active
    \def*{\kern\digitwidth}
    \newdimen\signwidth
    \setbox0=\hbox{-}
    \signwidth=\wd0
    \catcode`!=\active
    \def!{\kern\signwidth}
 \halign{
      \hbox to 1.5cm{#\leaderfil}\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      #\tabskip 0em\hfil\cr
    \noalign{\doubleline}
      \omit Band ID\hfil&
	\omit\hfil Detector Type \hfil&
      \omit\hfil Filter Construction \hfil\cr
      \noalign{\vskip 4pt\hrule\vskip 4pt}
      10 & Composite Si Bolometer & Sapphire/Grids/BaF$_2$/CsI/AgCl \cr
      *9 & Composite Si Bolometer & Sapphire/Mesh Grids/BaF$_2$/KBr  \cr
      *8 & Ge:Ga & MLIF/KCl/CaF$_2$/Sapphire \cr
      *7 & Ge:Ga & MLIF/Sapphire/KRS5/Crystal Quartz \cr
      *6 & Si:As BIB   &  MLIF/Silicon \cr
      *5 & Si:As BIB   & MLIF/Germanium/ZnSe \cr
      *4 & InSb &        MLIF/Germanium \cr
      *3 & InSb &        Coated Germanium \cr
      *2 & InSb &        Coated Glass \cr
      *1 & InSb &        Coated Glass \cr
      \noalign{\vskip 4pt\hrule\vskip 5pt} } }
  \endPlancktablewide \endgroup
\end{table*}


==> planet_flag_table.tex <==
\begin{table}[t]
  \begingroup
  \newdimen\tblskip \tblskip=5pt
	\caption{List of celestial body flags.}
  \label{tab:planet_flags}
  \nointerlineskip
  \vskip -3mm
  \footnotesize
  \setbox\tablebox=\vbox{
    \newdimen\digitwidth
    \setbox0=\hbox{\rm 0}
    \digitwidth=\wd0
    \catcode`*=\active
    \def*{\kern\digitwidth}
    \newdimen\signwidth
    \setbox0=\hbox{-}
    \signwidth=\wd0
    \catcode`!=\active
    \def!{\kern\signwidth}
 \halign{
      \hbox to 1.5cm{#\leaderfil}\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      #\tabskip 0em\hfil\cr
    \noalign{\doubleline}
      \omit Object\hfil&
      \omit\hfil Radius ($^\circ$) \hfil\cr
      \noalign{\vskip 4pt\hrule\vskip 4pt}
      Moon****** & 10 \cr
      Mercury*** & *1 \cr
      Venus***** & *2 \cr
      Mars****** & *2 \cr
      Jupiter*** & *2 \cr
      Saturn**** & *1 \cr
      Uranus**** & *1 \cr
      Neptune*** & *1 \cr
      \noalign{\vskip 4pt\hrule\vskip 5pt} } }
  \endPlancktablewide \endgroup
\end{table}


==> summary_table.tex <==
\begin{table*}[t]
  \begingroup
  \newdimen\tblskip \tblskip=5pt
  \caption{Key map-level characteristics of the \cosmoglobe\ DR2 ZSMA maps. The relative calibration, $\alpha$, is defined as the slope of a scatter plot between the old K98 and new DR2 maps, evaluated over either the default DR2 processing mask (``High latitudes'') or full sky. }
  \label{tab:summary}
  \nointerlineskip
  \vskip -3mm
  \footnotesize
  \setbox\tablebox=\vbox{
    \newdimen\digitwidth
    \setbox0=\hbox{\rm 0}
    \digitwidth=\wd0
    \catcode`*=\active
    \def*{\kern\digitwidth}
    \newdimen\signwidth
    \setbox0=\hbox{-}
    \signwidth=\wd0
    \catcode`!=\active
    \def!{\kern\signwidth}
 \halign{
      \hbox to 2.0cm{#\leaderfil}\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 2em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 2em&
      \hfil#\hfil\tabskip 1em&
      \hfil#\hfil\tabskip 0em\cr
      \noalign{\doubleline}
      \omit&\multispan3\hfil\sc Bandpass$^{(\mathrm{a})}$ \hfil&\multispan2\hfil\sc Relative calibration, $\alpha$ \hfil&\multispan2\hfil\sc Noise rms (kJy/sr)$^{(\mathrm{b})}$ \hfil\cr
\noalign{\vskip -3pt}
\omit&\multispan3\hrulefill&\multispan2\hrulefill&\multispan2\hrulefill\cr
\noalign{\vskip 3pt} 
\omit\sc Channel ID\hfil& $\nu_{\mathrm{c}}$ (THz) & $\lambda_{\mathrm{c}}$ ($\mu$m) & $\Delta\nu/\nu\hfil$ & High lat & Full sky & K98 & DR2 \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
      *1 & 240  & 1.25 & 0.25 &  1.025 & 1.068 & ***1.0 & ***1.3 \cr
      *2 & 136  & 2.2  & 0.16 &  1.022 & 1.034 & ***1.2 & ***1.8 \cr
      *3 & 85.7 & 3.5  & 0.26 &  1.012 & 1.031 & ***1.1 & ***1.5 \cr
      *4 & 61.2 & 4.9  & 0.13 &  0.974 & 1.028 & ***1.3 & ***1.3 \cr
      *5 & 25.0 & *12  & 0.53 &  0.629 & 0.943 & ***3.6 & **8.8 \cr
      *6 & 12.0 & *25  & 0.34 &  0.206 & 1.019 & ***7.5 & **15 \cr
      *7 & 5.00 & *60  & 0.46 &  1.009 & 0.988 & **18 & **18 \cr
      *8 & 3.00 & 100  & 0.32 &  1.005 & 1.041 & **17 & **19 \cr
      *9 & 2.14 & 140  & 0.28 &  0.784 & 1.013 & 1530 & 1270 \cr
      10 & 1.25 & 240  & 0.40 &  0.841 & 1.012 & *860 & *740 \cr
      \noalign{\vskip 4pt\hrule\vskip 5pt} } }
  \endPlancktablewide 
  \tablenote {{\rm a}} Reproduced from the DIRBE Explanatory Supplement.\par
  \tablenote {{\rm b}} Noise sensitivity per $0.7^{\circ}\times 0.7^{\circ}$ pixel, averaged over the full sky.\par
\endgroup
\end{table*}

